SOYO: A Tuning-Free Approach for Video Style Morphing via Style-Adaptive Interpolation in Diffusion Models

Diffusion models have achieved remarkable progress in image and video stylization. However, most existing methods focus on single-style transfer, while video stylization involving multiple styles necessitates seamless transitions between them. We refer to this smooth style transition between video frames as video style morphing. Current approaches often generate stylized video frames with discontinuous structures and abrupt style changes when handling such transitions. To address these limitations, we introduce SOYO, a novel diffusion-based framework for video style morphing. Our method employs a pre-trained text-to-image diffusion model without fine-tuning, combining attention injection and AdaIN to preserve structural consistency and enable smooth style transitions across video frames. Moreover, we notice that applying linear equidistant interpolation directly induces imbalanced style morphing. To harmonize across video frames, we propose a novel adaptive sampling scheduler operating between two style images. Extensive experiments demonstrate that SOYO outperforms existing methods in open-domain video style morphing, better preserving the structural coherence of video frames while achieving stable and smooth style transitions.

==> sec/3_method_soyo_beifen.tex <==
\section{Method}

Video Style Morphing refers to the task of generating a video $I'^{[1:N]}$ that maintains the structural consistency of a given input video $I^{[1:N]}$ while smoothly transitioning its visual style from the style of an image $I^{s0}$ to that of another image $I^{s1}$ over time. To address this challenging problem, we propose SOYO, a novel approach that leverages a pre-trained Text-to-Image (T2I) Stable Diffusion (SD) model to enable tuning-free Video Style Morphing. For simplicity, the subsequent discussion omits the details of the encoding and decoding processes of the latent diffusion model (LDM) autoencoder.


\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{figure/method.pdf} 
    \caption{SOYO pipeline. We perform DDIM Inversion on the source video $I^{[1:N]}$ to obtain $z^c_T$, and execute DDIM Inversion on two style images $I^{s0}$ and $I^{s1}$ to get $z^{s0}_T$ and $z^{s1}_T$, respectively, while saving their attention values.Subsequently, we perform linear interpolation on \( z^{s0}_t \) and \( z^{s1}_t \) with specific weights to obtain \( z^s_t \), which is then used to modulate \( z^c_t \) via AdaIN. During the denoising process, the latents corresponding to each frame are injected with interpolated $K^s$ and $V^s$ values from the style images, while receiving $Q^c$ injections from the source video frames. This results in smoothly transitioned stylized video frames $I'^{[1:N]}$.} 
    \label{fig:method} 
\end{figure*}

\subsection{Preliminary for Diffusion Models}

Diffusion models~\cite{ho2020denoising, song2020denoising} are probabilistic generative models that generate images through a gradual denoising process. The framework consists of two main phases: a \textit{forward} process that progressively adds Gaussian noise to the data, and a \textit{reverse} process that learns to denoise and recover the original data. During generation, the model starts with random noise and iteratively refines it, gradually producing a high-quality image through learned noise prediction.

Our method builds on the text-conditioned Stable Diffusion (SD) model~\cite{rombach2022high}, which performs denoising in a compact latent space to enhance efficiency. The pipeline first maps input images into this latent space using a VAE encoder~\cite{kingma2013auto}, applies the diffusion process and then decodes the refined latent representation back into the image space. In the noise-predicting network $\epsilon_{\theta}$, residual blocks generate intermediate features $f_t^l$, which are further processed using attention mechanisms.

Self-attention captures long-range spatial dependencies within the features:
\begin{equation}
    Attention(Q, K, V) = \text{softmax}\left(\frac{QK^\top}{\sqrt{d_k}}\right) \cdot V
\end{equation}
where $Q$, $K$, and $V$ represent queries, keys, and values derived from the same feature map, with $d_k$ indicating the key/query dimension.

Cross-attention integrates the textual prompt $P$ by using it to generate keys and values, thereby merging the semantics of both text and image. These attention layers in the SD model play a key role in guiding image composition and synthesis, enabling edits by manipulating attention during the denoising process.



\subsection{Cross-Frame Style Fusion Attention}
To ensure both temporal consistency and spatial coherence across the generated video frames, we extend the Latent Diffusion Model (LDM) into three-dimensional space. In this extension, we modify the self-attention mechanism to incorporate cross-frame attention, which is defined as follows:

\begin{equation}
\begin{aligned}
Q^i &= W^Q z^i, \\
K^i &= W^K [z^{i-1}, z^i, z^{i+1}], \\
V^i &= W^V [z^{i-1}, z^i, z^{i+1}].
\end{aligned}
\end{equation}

To mitigate the risk of overfitting to the style image, it is essential to ensure that stylized video frames derive structural information from the source video while acquiring textural details from the style image. Prior research in image and video editing has demonstrated that manipulating self-attention significantly influences the structural and textural properties of video frames. In our approach, we extract frame structures from the source video and frame textures from the style images, leveraging these features to guide the generation process. 

We begin by performing DDIM inversion on the source video to extract its self-attention (SA) features, denoted by $Q^c$, along with the corresponding noise term, $z_T^c$. Similarly, we apply DDIM inversion to the two style images to extract their respective SA features, $\{K^s_0, V^s_0\}$ and $\{K^s_1, V^s_1\}$, as well as their noise terms $z_T^{s_0}$ and $z_T^{s_1}$. These features are injected during the denoising process. The query features, \( Q_t \), play a critical role in capturing the structural characteristics of the generated video frames. Given that structural features are essential throughout the denoising process, we continuously incorporate the features \( Q^c \) from the source video at each denoising stage. By directly setting \( Q_t = Q^c_t \) across all timesteps, we ensure the consistent preservation of the structural elements from the source video throughout the entire process. This approach safeguards the structural integrity of the source video, while textural aspects are managed separately through the key and value features.


In contrast to previous approaches that inject self-attention features from a single style image, our method generates intermediate transitional states by adaptively interpolating both the key (\( K \)) and value (\( V \)) features from the self-attention layers of two distinct style images, as illustrated in Fig. \ref{fig:injection}. These hybrid features, which dictate the textural synthesis of the generated frames, are progressively integrated during the denoising process to ensure smooth stylistic transitions. Specifically, the interpolated matrices \( K^m \) and \( V^m \) blend complementary visual patterns from both source styles, facilitating a continuous and coherent temporal fusion between the two artistic expressions throughout the frame generation pipeline.



\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figure/injection.pdf} 
    \caption{The injection of keys and values derived from a single style image results in stylized video frames that fail to accurately represent the desired textures and transitions. This issue can be effectively addressed by performing linear interpolation between the keys and values corresponding to two distinct style images.} 
    \label{fig:injection} 
\end{figure}



\begin{equation}
\begin{aligned}
K^m_t &= \text{LinearInterp}(K^s_{0,t}, K^s_{1,t}, \alpha), \\
V^m_t &= \text{LinearInterp}(V^s_{0,t}, V^s_{1,t}, \alpha),
\end{aligned}
\end{equation}

Where  $\alpha$ represents interpolation coefficients that control the gradual transition between the two style images. The modified self-attention process is calculated as follows: 

\begin{equation}
    Attention(Q^c_t, K^m_t, V^m_t) = \text{softmax}\left(\frac{{Q^c_t(K^m_t)}^\top}{\sqrt{d_k}}\right)\cdot V^m_t
\end{equation}

This approach ensures that the structural integrity of the source video is preserved across all frames, while still allowing the style to be gradually infused through the interpolated $K$ and $V$ features, leading to temporally coherent and stylistically consistent results.





\subsection{Dual-Style Latent AdaIN Modulation}

In style transfer tasks, preserving the consistency of color tones and brightness is essential when transferring style information from reference images to target video frames. To ensure this, we employ the Adaptive Instance Normalization (AdaIN)~\cite{huang2017arbitrary} technique, which adjusts the latent representations of the target frames by modulating them with the style statistics (mean and standard deviation) extracted from the reference images.

In video style morphing, where the objective is to gradually transition the visual style of a video from one reference image to another, we interpolate between the mean and standard deviation of the latents derived from the two reference images. This interpolation is governed by a time-dependent parameter \( \alpha \), which adaptively controls the degree of style blending between the two reference styles across the video frames, ensuring a smooth and continuous stylistic transition.


Let \( z_t^c \) denote the latent features of the target video frame, and let \( z_t^{s0} \) and \( z_t^{s1} \) represent the latents derived from the two reference images. The first step is to compute the mean \( \mu \) and standard deviation \( \sigma \) of these latents. The interpolated mean \( \mu_t^s \) and standard deviation \( \sigma_t^s \) for the style transfer are then computed as a weighted average between the two reference latents:

\begin{equation}
    \mu_t^s = \alpha \cdot \mu(z_t^{s0}) + (1 - \alpha) \cdot \mu(z_t^{s1})
\end{equation}

\begin{equation}
    \sigma_t^s = \alpha \cdot \sigma(z_t^{s0}) + (1 - \alpha) \cdot \sigma(z_t^{s1})
\end{equation}

Here, \( \alpha \) is the interpolation coefficient, which starts at 0 for the first frame, corresponding to the style of the first reference image, and gradually increases to 1 as the video progresses, transitioning towards the style of the second reference image. 

The AdaIN modulation is then applied to the target video frame latents \( z_t^c \) using the interpolated style statistics \( \mu_t^s \) and \( \sigma_t^s \):

\begin{equation}
    z_t = \sigma_t^s \left( \frac{z_t^c - \mu(z_t^c)}{\sigma(z_t^c) + \epsilon} \right) + \mu_t^s
\end{equation}

Where \( \mu(z_t^c) \) and \( \sigma(z_t^c) \) represent the mean and standard deviation of the target video frame latent \( z_t^c \), and \( \epsilon \) is a small constant added to avoid division by zero. This operation ensures that the generated video frame \( z_t \) is stylized with the desired visual features while preserving the structural consistency of the original content.

By progressively modulating the interpolation coefficient \( \alpha \) throughout the video sequence, we achieve a seamless transition between the two reference styles, ensuring both temporal coherence and stylistic fidelity. This approach enables a smooth and continuous evolution of style across video frames, preserving the structural integrity of the target content while adapting its color and texture characteristics to align with the desired reference styles.



 



 
\subsection{Adaptive Style Distance Mapping}

To address the issue of imbalanced style transformation in video style transfer, where specific style pairs lead to asymmetric transitions—resulting in a slower style change on one side and more than half of the frames being biased toward a particular style—we propose a balanced control method, Adaptive Style Distance Mapping (ASDM), implemented as follows. 
First, we perform pre-sampling from the 10th denoising step to rapidly generate a set of stylized frames. These frames are then processed through a pre-trained VGG16 network~\cite{simonyan2014very} to compute the style distance, which is measured by the differences in mean and standard deviation at various feature layers between the generated frames and the two reference style images. Based on these distance curves, we identify the perceptual style transition point, denoted as \( \alpha_{\text{mid}} \), and normalize it according to the total number of frames. 
Next, we construct a baseline linear transition curve for \( \alpha \) using \( \texttt{LinSpace}(0,1) \) over all frames. To emphasize regions where perceptual style change is more pronounced, we introduce an adaptive scaling factor, defined as 

\begin{equation}
S_{\text{max}} = 1 + \lambda_{\alpha} \,|\alpha_{\text{mid}} - 0.5|.
\end{equation}

If \( \alpha_{\text{mid}} < 0.5 \), the scaling factor is gradually increased from 1 to \( S_{\text{max}} \); otherwise, it decreases from \( S_{\text{max}} \) back to 1. The differences between consecutive values in the baseline curve are then modulated by these scaling factors, and their cumulative sum—normalized to the range \([0,1]\)—produces a non-uniform \( \alpha \) curve. This adaptive mapping ensures a higher sampling density in regions with more significant perceptual style changes, leading to a smoother and visually balanced style transition throughout the video.


==> sec/7_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/8_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
